Semirandom Planted Clique and the Restricted Isometry Property

We give a simple, greedy $O(n^{\omega+0.5})=O(n^{2.872})$-time algorithm to list-decode planted cliques in a semirandom model introduced in [CSV17] (following [FK01]) that succeeds whenever the size of the planted clique is $k\geq O(\sqrt{n} \log^2 n)$. In the model, the edges touching the vertices in the planted $k$-clique are drawn independently with probability $p=1/2$ while the edges not touching the planted clique are chosen by an adversary in response to the random choices. Our result shows that the computational threshold in the semirandom setting is within a $O(\log^2 n)$ factor of the information-theoretic one [Ste17] thus resolving an open question of Steinhardt. This threshold also essentially matches the conjectured computational threshold for the well-studied special case of fully random planted clique. All previous algorithms [CSV17, MMT20, BKS23] in this model are based on rather sophisticated rounding algorithms for entropy-constrained semidefinite programming relaxations and their sum-of-squares strengthenings and the best known guarantee is a $n^{O(1/\epsilon)}$-time algorithm to list-decode planted cliques of size $k \geq \tilde{O}(n^{1/2+\epsilon})$. In particular, the guarantee trivializes to quasi-polynomial time if the planted clique is of size $O(\sqrt{n} \operatorname{polylog} n)$. Our algorithm achieves an almost optimal guarantee with a surprisingly simple greedy algorithm. The prior state-of-the-art algorithmic result above is based on a reduction to certifying bounds on the size of unbalanced bicliques in random graphs -- closely related to certifying the restricted isometry property (RIP) of certain random matrices and known to be hard in the low-degree polynomial model. Our key idea is a new approach that relies on the truth of -- but not efficient certificates for -- RIP of a new class of matrices built from the input graphs.

==> rip.tex <==
\section{Restricted isometry property}
\label{sec:rip}
One of the main tools used in the analysis of our algorithm is a strong general theorem guaranteeing RIP for any matrix with independent rows drawn from any isotropic-distribution vectors with bounded entries.


\Cref{thm:rip}, although known, is usually stated in terms of so-called \emph{bounded orthonormal systems}, a formulation that makes its direct applicability in situations like~\Cref{lem:tensoring-gives-RIP} less transparent. 
For completeness, we introduce the notion of bounded orthonormal system, the formulation of~\Cref{thm:rip} as it is stated in \cite{MR2731597-Rauhut10}, and we discuss why this is equivalent to the statement we are using in this paper.

\begin{definition}
\label{def:bos}
A bounded orthonormal system is given by a region $\mathcal{D} \subset \R^k$, together with a probability measure $\mu$ on $\mathcal{D}$ and $N$ functions $\phi_1,\phi_2, \ldots \phi_d : \mathcal{D} \to \C$ satisfying the following properties:
\begin{itemize}
\item For all $i\not=j$ in $[N]$,
$\E_{t \sim \mu} \phi_i(t) \overline{\phi_j(t)} = 0$,
\item For all $i\in [N]$,
$\E_{t \sim \mu} \phi_i(t) = 0, \E_{t\sim \mu} |\phi_i(t)|^2 = 1$,
\item For all $i\in [N]$, $|\phi_i(t)| \leq K$ almost surely.
\end{itemize}
\end{definition}
Then Theorem 12.31 in \cite{FR13} (originally proved in~\cite{MR2417886-Rudelson08}) states:
\begin{theorem}[Theorem 12.31 in \cite{FR13}]
\label{thm:rip-bos}
If $\phi_1, \ldots, \phi_N$ together with a distribution $\mu$ is a bounded orthonormal system, then a matrix $H \in \C^{m \times N}$ obtained by sampling $t_1, t_2 \ldots t_m$ independently at random according to $\mu$ and setting $H_{i,j} = \phi_j(t_i)/\sqrt{m}$ satisfies $(r,\delta)$-RIP with probability $1-N^{-\log^3(r)}$ whenever
\begin{equation*}
m \gtrsim K^2 r \log^3 r \log(N) / \delta^2\,.
\end{equation*}
\end{theorem}
To see how this theorem implies \Cref{thm:rip}, let us consider an arbitrary distribution $\mu$ over $\R^n$ satisfying $\E_{\mathbf{X} \sim \mu} \mathbf{X} \mathbf{X}^\top = I$. We can take $\phi_1, \ldots \phi_N : \R^n \to \R$ such that $\phi_j$ is a projection on the $j$-th coordinate. Then $\phi_1, \ldots \phi_N$ together with the distribution $\mu$ forms a bounded orthonormal system according to \Cref{def:bos}, and the matrix $H_{i,j} = \phi_j(t_i)$ is exactly obtained by drawing $m$ independent random rows according to the law of $\mathbf{X}$.

The other direction of the equivalence (in the case of real-valued bounded orthonormal system) is just as immediate: if $\phi_1, \ldots, \phi_N$ together with $\mu$ form a bounded orthonormal system, then a random vector $\mathbf{X}$ obtained by drawing $t \sim \mu$ and setting $\mathbf{X} = (\phi_1(t), \ldots \phi_N(t))$ is a bounded vector in isotropic position.


